Knapsack Voting for Participatory Budgeting

We address the question of aggregating the preferences of voters in the context of participatory budgeting. We scrutinize the voting method currently used in practice, underline its drawbacks, and introduce a novel scheme tailored to this setting, which we call "Knapsack Voting". We study its strategic properties - we show that it is strategy-proof under a natural model of utility (a dis-utility given by the $\ell_1$ distance between the outcome and the true preference of the voter), and "partially" strategy-proof under general additive utilities. We extend Knapsack Voting to more general settings with revenues, deficits or surpluses, and prove a similar strategy-proofness result. To further demonstrate the applicability of our scheme, we discuss its implementation on the digital voting platform that we have deployed in partnership with the local government bodies in many cities across the nation. From voting data thus collected, we present empirical evidence that Knapsack Voting works well in practice.

==> mydefs.tex <==
%%%%%%%%% begin - my new commands/definitions %%%%%%%%%%%%%%%%%%%%%
\makeatletter
\DeclareRobustCommand{\qed}{%
  \ifmmode % if math mode, assume display: omit penalty etc.
  \else \leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
  \fi
  \quad\hbox{\qedsymbol}}
\newcommand{\openbox}{\leavevmode
  \hbox to.77778em{%
  \hfil\vrule
  \vbox to.675em{\hrule width.6em\vfil\hrule}%
  \vrule\hfil}}
\newcommand{\qedsymbol}{\openbox}
\newenvironment{proof}[1][\proofname]{\par
  \normalfont
  \topsep6\p@\@plus6\p@ \trivlist
  \item[\hskip\labelsep\itshape
    #1.]\ignorespaces
}{%
  \qed\endtrivlist
}
\newcommand{\proofname}{Proof}
\makeatother

\newtheorem{lemma}{Lemma}[section]
\newtheorem{problem}{Problem}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{observation}{Observation}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{note}{Note}[section]
\newtheorem{hypothesis}{Empirical Hypothesis}[section]
\newtheorem{lp}{Linear Program}[section]
\newtheorem{result}{Result}[section]
\newtheorem{example}{Example}[section]
\newcommand{\C}{\mathcal{C}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\p}{\mathcal{P}}
\newcommand{\pp}{\mathcal{P}^\prime}
\newcommand{\rr}{\mathcal{R}^\prime}
\newcommand{\ppp}{p^\prime}
\newcommand{\sss}{S_i^{\star\star}}
\newcommand{\vp}{v^\prime}
\newcommand{\W}{\mathcal{W}}
\newcommand{\indicator}{\mathbbm{1}}
\newcommand{\score}{\mathrm{score}}

%\newcommand{\h}{\mathcal{H}}
%\newcommand{\m}{\mathcal{M}}
%\newcommand{\nnreals}{\mathbb R_{\ge 0}}
%\newcommand{\nnints}{\mathbb Z_{\ge 0}}
%\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}
%\newcommand{\otherstodo}{\color{blue}}
%\newcommand{\mytodo}{\color{red}}
%%%%%%%%% \end - my new commands/definitions %%%%%%%%%%%%%%%%%%%%%
\usepackage{bbm}
\usepackage{color}
\newcommand{\markit}{$\spadesuit$}
%\usepackage{caption}
%\usepackage{subcaption}
%\newenvironment{oneshot}[1]{\@begintheorem{#1}{\unskip}}{\@endtheorem}
